A Moral Framework for Understanding of Fair ML through Economic Models of Equality of Opportunity

We map the recently proposed notions of algorithmic fairness to economic models of Equality of opportunity (EOP)---an extensively studied ideal of fairness in political philosophy. We formally show that through our conceptual mapping, many existing definition of algorithmic fairness, such as predictive value parity and equality of odds, can be interpreted as special cases of EOP. In this respect, our work serves as a unifying moral framework for understanding existing notions of algorithmic fairness. Most importantly, this framework allows us to explicitly spell out the moral assumptions underlying each notion of fairness, and interpret recent fairness impossibility results in a new light. Last but not least and inspired by luck egalitarian models of EOP, we propose a new family of measures for algorithmic fairness. We illustrate our proposal empirically and show that employing a measure of algorithmic (un)fairness when its underlying moral assumptions are not satisfied, can have devastating consequences for the disadvantaged group's welfare.

==> table.tex <==
\paragraph{Tradeoffs among Various Measures of Fairness}
Finally, we demonstrate the existence of multilateral tensions among accuracy, social welfare, individual, and statistical measures of (un)fairness by looking at the predictive models that would optimize each. See Table~\ref{tab:opt}. In the realizable case, we assume the existence of a hypothesis $h^* \in \cH$ such that $y = h^*(\vx)$ (perfect prediction accuracy); for the unrealizable case, we assume the existence of a hypothesis $h^* \in \cH$, such that $h^*(\vx) = \Exp[y|\vx])$. Also we define $y_{\text{max}} = \max_{h \in \cH , \vx \in \cX} h(\vx)$ and $y_{\text{min}} = \min_{h \in \cH , \vx \in \cX} h(\vx)$.
\begin{table}[h!]
  \caption{Optimal predictions with respect to different notions of fairness}
  \label{tab:opt}
  { \small
	\begin{tabular}{  c | c | c | c | c |}
  		\cline{2-5}
   	& \multicolumn{2}{c|}{Classification} & \multicolumn{2}{c |}		{Regression}\\
	  \cline{2-5}
   		& Realizable & Unrealizable  & Realizable & Unrealizable \\
  \hline
%  \multicolumn{1}{|c|}{Loss} & $\hy = h^*(\vx)$ & $\hy = \ones [h^*(\vx)\geq 0.5]$ & $\hy = h^*(\vx)$ & $\hy = h^*(\vx)$ \\ \cline{1-1}
  \multicolumn{1}{|c|}{Social welfare} & $\hy \equiv 1$ & $\hy \equiv 1$ & $\hy \equiv y_{\text{max}}$ & $\hy \equiv y_{\text{max}}$ \\ \cline{1-1}
  \multicolumn{1}{|c|}{Atkinson index} & $\hy = h^*(\vx)$ & $\hy \equiv 1$ & $\hy = h^*(\vx)$ & $\hy \equiv y_{\text{max}}$ \\ \cline{1-1}
  \multicolumn{1}{|c|}{Dwork et al.}  & $\hy \equiv 0$ or $1$ & $\hy \equiv 1$ or $0$ & $\hy \equiv c$ & $\hy \equiv c$ \\ \cline{1-1}
  \multicolumn{1}{|c|}{Mean diff.} & $\hy \equiv 0$ or $1$ & $\hy \equiv 1$ or $0$ & $\hy \equiv c$ & $\hy \equiv c$ \\ \cline{1-1}
  \multicolumn{1}{|c|}{Pos. res. diff.} & $\hy \equiv 0$ or $\hy = h^*(\vx)$ & $\hy \equiv 0$ & $\hy \equiv y_{\text{min}}$ or $\hy = h^*(\vx)$& $\hy \equiv y_{\text{min}}$ \\ \cline{1-1}
  \multicolumn{1}{|c|}{Neg. res. diff.} & $\hy \equiv 1$ or $\hy = h^*(\vx)$ & $\hy \equiv 1$ & $\hy \equiv y_{\text{max}}$ or $\hy = h^*(\vx)$ & $\hy \equiv y_{\text{max}}$ \\ \cline{1-1}
  \hline
\end{tabular}}
\end{table}

To see the tradeoffs among various notions of fairness, and between accuracy and fairness, take the unrealizable classification case as an example. Optimizing for accuracy obviously requires the predictions to follow the Bayes optimal classifier. On the one hand, a lower bound on social welfare pulls the model in the direction of allocating the desirable outcome (i.e. 1) to a larger fraction of the population. On the other hand, to guarantee low positive residual difference, individuals should ideally all receive a label less than their ground truth (e.g. 0).

